RG-CAT: Detection Pipeline and Catalogue of Radio Galaxies in the EMU Pilot Survey

We present source detection and catalogue construction pipelines to build the first catalogue of radio galaxies from the 270 $\rm deg^2$ pilot survey of the Evolutionary Map of the Universe (EMU-PS) conducted with the Australian Square Kilometre Array Pathfinder (ASKAP) telescope. The detection pipeline uses Gal-DINO computer-vision networks (Gupta et al., 2024) to predict the categories of radio morphology and bounding boxes for radio sources, as well as their potential infrared host positions. The Gal-DINO network is trained and evaluated on approximately 5,000 visually inspected radio galaxies and their infrared hosts, encompassing both compact and extended radio morphologies. We find that the Intersection over Union (IoU) for the predicted and ground truth bounding boxes is larger than 0.5 for 99% of the radio sources, and 98% of predicted host positions are within $3^{\prime \prime}$ of the ground truth infrared host in the evaluation set. The catalogue construction pipeline uses the predictions of the trained network on the radio and infrared image cutouts based on the catalogue of radio components identified using the Selavy source finder algorithm. Confidence scores of the predictions are then used to prioritize Selavy components with higher scores and incorporate them first into the catalogue. This results in identifications for a total of 211,625 radio sources, with 201,211 classified as compact and unresolved. The remaining 10,414 are categorized as extended radio morphologies, including 582 FR-I, 5,602 FR-II, 1,494 FR-x (uncertain whether FR-I or FR-II), 2,375 R (single-peak resolved) radio galaxies, and 361 with peculiar and other rare morphologies. We cross-match the radio sources in the catalogue with the infrared and optical catalogues, finding infrared cross-matches for 73% and photometric redshifts for 36% of the radio galaxies.

==> tables/table_2.tex <==
\begin{tabular}{rlllllllllll}
\toprule
 GalDINO\_n\_selavy\_components &                                   selavy\_island\_id &                                selavy\_component\_id &                              selavy\_component\_name &                         selavy\_ra\_hms\_cont &                     selavy\_dec\_hms\_cont &                  selavy\_ra\_deg\_cont &                  selavy\_dec\_deg\_cont &                                      selavy\_ra\_err &                                     selavy\_dec\_err &                                   selavy\_flux\_peak &                               selavy\_flux\_peak\_err \\
\midrule
                           1 &                                SB9287\_island\_73247 &                            SB9287\_component\_73247b &                                     J203428-583922 &                                 20:34:28.9 &                               -58:39:22 &                          308.620413 &                           -58.656166 &                                 0.7099999785423279 &                                 1.6299999952316284 &                                0.11100000143051147 &                              0.0020000000949949026 \\
                           3 & ['SB9287\_island\_51392', 'SB9287\_island\_51392', ... & ['SB9287\_component\_51392c', 'SB9287\_component\_5... & ['J210453-544712', 'J210450-544723', 'J210449-5... & ['21:04:53.2', '21:04:50.5', '21:04:49.4'] & ['-54:47:12', '-54:47:23', '-54:46:51'] & [316.221701, 316.21049, 316.205665] & [-54.786732, -54.789826, -54.780905] & [0.1599999964237213, 0.05999999865889549, 0.079... & [0.07000000029802322, 0.11999999731779099, 0.14... & [0.3190000057220459, 0.5199999809265137, 0.3610... & [0.003000000026077032, 0.003000000026077032, 0.... \\
                           1 &                                 SB9287\_island\_6828 &                             SB9287\_component\_6828a &                                     J202025-604829 &                                 20:20:25.6 &                               -60:48:29 &                          305.106637 &                           -60.808267 &                               0.009999999776482582 &                               0.009999999776482582 &                                  6.873000144958496 &                                0.00800000037997961 \\
                           1 &                                SB9287\_island\_20187 &                            SB9287\_component\_20187a &                                     J201051-604912 &                                 20:10:51.5 &                               -60:49:12 &                          302.714398 &                           -60.820226 &                                0.03999999910593033 &                                0.03999999910593033 &                                  1.659000039100647 &                               0.006000000052154064 \\
                           1 &                               SB9287\_island\_144030 &                           SB9287\_component\_144030a &                                     J221710-591718 &                                 22:17:10.3 &                               -59:17:18 &                          334.293099 &                           -59.288521 &                                0.07999999821186066 &                                0.07000000029802322 &                                 0.2070000022649765 &                              0.0020000000949949026 \\
                           1 &                               SB9287\_island\_118230 &                           SB9287\_component\_118230a &                                     J211549-530854 &                                 21:15:49.3 &                               -53:08:54 &                          318.955529 &                           -53.148423 &                                0.17000000178813934 &                                 0.2199999988079071 &                                 0.2329999953508377 &                               0.004000000189989805 \\
                           1 &                               SB9287\_island\_153701 &                           SB9287\_component\_153701a &                                     J203404-622500 &                                 20:34:04.9 &                               -62:25:00 &                          308.520296 &                           -62.416735 &                                0.07000000029802322 &                                               0.25 &                                0.18799999356269836 &                               0.004000000189989805 \\
                           1 &                               SB9287\_island\_121092 &                           SB9287\_component\_121092a &                                     J220545-502550 &                                 22:05:45.7 &                               -50:25:50 &                           331.44024 &                           -50.430578 &                                0.05000000074505806 &                                0.05000000074505806 &                                 0.2460000067949295 &                              0.0020000000949949026 \\
                           1 &                                SB9287\_island\_90811 &                            SB9287\_component\_90811a &                                     J220957-493722 &                                 22:09:57.8 &                               -49:37:22 &                          332.490668 &                           -49.623007 &                                 0.3499999940395355 &                                0.15000000596046448 &                                 0.2759999930858612 &                               0.004999999888241291 \\
                           1 &                               SB9287\_island\_161723 &                           SB9287\_component\_161723a &                                     J215754-561007 &                                 21:57:54.2 &                               -56:10:07 &                          329.476016 &                           -56.168736 &                                0.28999999165534973 &                                0.38999998569488525 &                                0.16699999570846558 &                               0.003000000026077032 \\
                           1 &                               SB9287\_island\_138293 &                           SB9287\_component\_138293a &                                     J203010-513900 &                                 20:30:10.8 &                               -51:39:00 &                           307.54483 &                           -51.650187 &                                0.07000000029802322 &                                0.07000000029802322 &                                0.21699999272823334 &                              0.0020000000949949026 \\
                           1 &                               SB9287\_island\_109116 &                           SB9287\_component\_109116a &                                     J215126-541420 &                                 21:51:26.8 &                               -54:14:20 &                          327.861684 &                           -54.238972 &                               0.019999999552965164 &                               0.019999999552965164 &                                 0.2680000066757202 &                              0.0010000000474974513 \\
                           1 &                               SB9287\_island\_144691 &                           SB9287\_component\_144691a &                                     J214906-583402 &                                 21:49:06.1 &                               -58:34:02 &                          327.275235 &                            -58.56746 &                                0.03999999910593033 &                                0.03999999910593033 &                                0.20900000631809235 &                              0.0010000000474974513 \\
                           1 &                               SB9287\_island\_168768 &                           SB9287\_component\_168768a &                                     J211916-544326 &                                 21:19:16.8 &                               -54:43:26 &                          319.819837 &                           -54.723968 &                               0.029999999329447746 &                               0.029999999329447746 &                                0.18299999833106995 &                              0.0010000000474974513 \\
                           1 &                                SB9287\_island\_26036 &                            SB9287\_component\_26036a &                                     J205252-621232 &                                 20:52:52.6 &                               -62:12:32 &                           313.21913 &                           -62.208975 &                               0.019999999552965164 &                               0.019999999552965164 &                                 1.1610000133514404 &                               0.004000000189989805 \\
                           1 &                               SB9287\_island\_179729 &                           SB9287\_component\_179729a &                                     J210642-583553 &                                 21:06:42.1 &                               -58:35:53 &                          316.675545 &                           -58.598192 &                                0.05000000074505806 &                                0.07000000029802322 &                                0.16500000655651093 &                              0.0010000000474974513 \\
                           1 &                                SB9287\_island\_10909 &                            SB9287\_component\_10909a &                                     J221750-581022 &                                 22:17:50.1 &                               -58:10:22 &                          334.458621 &                           -58.172934 &                               0.019999999552965164 &                               0.019999999552965164 &                                  3.740999937057495 &                               0.008999999612569809 \\
                           1 &                               SB9287\_island\_132561 &                           SB9287\_component\_132561a &                                     J215806-562514 &                                 21:58:06.8 &                               -56:25:14 &                          329.528216 &                           -56.420732 &                               0.019999999552965164 &                               0.019999999552965164 &                                0.23100000619888306 &                              0.0010000000474974513 \\
                           1 &                                SB9287\_island\_65564 &                            SB9287\_component\_65564a &                                     J221455-552441 &                                 22:14:55.8 &                               -55:24:41 &                          333.732575 &                           -55.411511 &                               0.029999999329447746 &                                0.03999999910593033 &                                 0.4129999876022339 &                              0.0020000000949949026 \\
                           1 &                               SB9287\_island\_100377 &                           SB9287\_component\_100377a &                                     J212155-575239 &                                 21:21:55.8 &                               -57:52:39 &                          320.482363 &                            -57.87755 &                               0.019999999552965164 &                               0.019999999552965164 &                                 0.2879999876022339 &                              0.0010000000474974513 \\
                           1 &                               SB9287\_island\_128086 &                           SB9287\_component\_128086a &                                     J203015-591223 &                                 20:30:15.8 &                               -59:12:23 &                          307.565975 &                           -59.206409 &                               0.029999999329447746 &                               0.029999999329447746 &                                0.23399999737739563 &                              0.0010000000474974513 \\
                           1 &                                SB9287\_island\_86236 &                            SB9287\_component\_86236a &                                     J211618-512747 &                                 21:16:18.0 &                               -51:27:47 &                          319.074929 &                           -51.463329 &                               0.029999999329447746 &                               0.029999999329447746 &                                0.33000001311302185 &                              0.0010000000474974513 \\
                           1 &                               SB9287\_island\_122350 &                           SB9287\_component\_122350a &                                     J211259-600829 &                                 21:12:59.1 &                               -60:08:29 &                          318.246151 &                           -60.141607 &                                0.03999999910593033 &                               0.029999999329447746 &                                0.24300000071525574 &                              0.0010000000474974513 \\
                           1 &                               SB9287\_island\_149394 &                           SB9287\_component\_149394a &                                     J202826-604530 &                                 20:28:26.1 &                               -60:45:30 &                          307.108886 &                           -60.758369 &                                0.07000000029802322 &                                0.05000000074505806 &                                0.20499999821186066 &                              0.0010000000474974513 \\
                           1 &                               SB9287\_island\_139208 &                           SB9287\_component\_139208a &                                     J221430-514837 &                                 22:14:30.0 &                               -51:48:37 &                          333.625201 &                           -51.810317 &                               0.029999999329447746 &                               0.029999999329447746 &                                0.21799999475479126 &                              0.0010000000474974513 \\
                           1 &                                 SB9287\_island\_4003 &                             SB9287\_component\_4003a &                                     J210804-505451 &                                 21:08:04.4 &                               -50:54:51 &                          317.018284 &                           -50.914365 &                                                0.0 &                                                0.0 &                                 13.437000274658203 &                               0.004999999888241291 \\
                           1 &                               SB9287\_island\_170120 &                           SB9287\_component\_170120a &                                     J211409-515338 &                                 21:14:09.8 &                               -51:53:38 &                          318.540852 &                           -51.893934 &                                0.03999999910593033 &                                0.03999999910593033 &                                0.17900000512599945 &                              0.0010000000474974513 \\
                           1 &                                 SB9287\_island\_6088 &                             SB9287\_component\_6088a &                                     J200756-530904 &                                 20:07:56.5 &                               -53:09:04 &                          301.985527 &                           -53.151233 &                               0.009999999776482582 &                               0.009999999776482582 &                                  8.076000213623047 &                               0.006000000052154064 \\
                           1 &                               SB9287\_island\_164228 &                           SB9287\_component\_164228a &                                     J212726-504104 &                                 21:27:26.1 &                               -50:41:04 &                          321.858861 &                           -50.684554 &                               0.029999999329447746 &                                0.03999999910593033 &                                0.18700000643730164 &                              0.0010000000474974513 \\
                           1 &                               SB9287\_island\_187721 &                           SB9287\_component\_187721a &                                     J212137-573451 &                                 21:21:37.0 &                               -57:34:51 &                          320.404283 &                           -57.580941 &                                0.05000000074505806 &                                0.05999999865889549 &                                0.15299999713897705 &                              0.0010000000474974513 \\
                           1 &                                SB9287\_island\_14169 &                            SB9287\_component\_14169a &                                     J204815-513212 &                                 20:48:15.5 &                               -51:32:12 &                          312.064596 &                           -51.536937 &                               0.009999999776482582 &                               0.009999999776482582 &                                  2.611999988555908 &                              0.0020000000949949026 \\
                           1 &                               SB9287\_island\_117740 &                           SB9287\_component\_117740a &                                     J210744-592847 &                                 21:07:44.8 &                               -59:28:47 &                          316.936794 &                           -59.479976 &                                0.03999999910593033 &                                0.05000000074505806 &                                0.24799999594688416 &                              0.0010000000474974513 \\
                           1 &                               SB9287\_island\_173664 &                           SB9287\_component\_173664a &                                     J201956-514135 &                                 20:19:56.1 &                               -51:41:35 &                          304.983572 &                           -51.693124 &                                0.27000001072883606 &                                 0.1899999976158142 &                                0.16200000047683716 &                               0.003000000026077032 \\
                           1 &                                SB9287\_island\_87665 &                            SB9287\_component\_87665a &                                     J221338-485036 &                                 22:13:38.0 &                               -48:50:36 &                          333.408262 &                           -48.843516 &                                0.05000000074505806 &                                0.05000000074505806 &                                 0.3269999921321869 &                              0.0020000000949949026 \\
                           1 &                               SB9287\_island\_167807 &                           SB9287\_component\_167807b &                                     J203815-562657 &                                 20:38:15.3 &                               -56:26:57 &                          309.563904 &                           -56.449426 &                                0.07999999821186066 &                                0.07000000029802322 &                                0.13300000131130219 &                              0.0010000000474974513 \\
                           1 &                               SB9287\_island\_177529 &                           SB9287\_component\_177529a &                                     J204010-550441 &                                 20:40:10.6 &                               -55:04:41 &                          310.044107 &                           -55.078165 &                                0.03999999910593033 &                                0.05000000074505806 &                                0.17100000381469727 &                              0.0010000000474974513 \\
                           1 &                               SB9287\_island\_161503 &                           SB9287\_component\_161503a &                                     J215753-572734 &                                 21:57:53.6 &                               -57:27:34 &                          329.473439 &                           -57.459654 &                                0.03999999910593033 &                                0.03999999910593033 &                                0.18799999356269836 &                              0.0010000000474974513 \\
                           1 &                               SB9287\_island\_105884 &                           SB9287\_component\_105884a &                                     J214544-532821 &                                 21:45:44.6 &                               -53:28:21 &                          326.435663 &                           -53.472738 &                               0.019999999552965164 &                               0.019999999552965164 &                                 0.2770000100135803 &                              0.0010000000474974513 \\
                           1 &                                SB9287\_island\_75350 &                            SB9287\_component\_75350a &                                     J213251-614021 &                                 21:32:51.6 &                               -61:40:21 &                           323.21486 &                           -61.672624 &                               0.029999999329447746 &                               0.029999999329447746 &                                 0.3709999918937683 &                              0.0010000000474974513 \\
                           1 &                                SB9287\_island\_11917 &                            SB9287\_component\_11917b &                                     J211247-512452 &                                 21:12:47.9 &                               -51:24:52 &                          318.199726 &                           -51.414444 &                                0.07000000029802322 &                                0.07000000029802322 &                                 1.2100000381469727 &                               0.010999999940395355 \\
                           1 &                                SB9287\_island\_51331 &                            SB9287\_component\_51331a &                                     J220711-531742 &                                 22:07:11.3 &                               -53:17:42 &                           331.79717 &                           -53.295276 &                               0.019999999552965164 &                               0.019999999552965164 &                                 0.5370000004768372 &                              0.0010000000474974513 \\
                           1 &                                SB9287\_island\_57117 &                            SB9287\_component\_57117a &                                     J211025-583054 &                                 21:10:25.2 &                               -58:30:54 &                          317.605004 &                           -58.515271 &                               0.029999999329447746 &                               0.029999999329447746 &                                 0.4790000021457672 &                              0.0020000000949949026 \\
                           1 &                               SB9287\_island\_146310 &                           SB9287\_component\_146310a &                                     J205246-492527 &                                 20:52:46.0 &                               -49:25:27 &                          313.191793 &                           -49.424283 &                                0.07999999821186066 &                                0.17000000178813934 &                                 0.1899999976158142 &                               0.003000000026077032 \\
                           1 &                                SB9287\_island\_24793 &                            SB9287\_component\_24793a &                                     J215141-630100 &                                 21:51:41.8 &                               -63:01:00 &                          327.924225 &                           -63.016394 &                               0.029999999329447746 &                               0.029999999329447746 &                                 1.2480000257492065 &                               0.004000000189989805 \\
                           1 &                                SB9287\_island\_94866 &                            SB9287\_component\_94866a &                                     J202618-495343 &                                 20:26:18.8 &                               -49:53:43 &                           306.57854 &                           -49.895291 &                               0.029999999329447746 &                               0.029999999329447746 &                                0.30300000309944153 &                              0.0010000000474974513 \\
                           1 &                               SB9287\_island\_174948 &                           SB9287\_component\_174948a &                                     J220537-562103 &                                 22:05:37.1 &                               -56:21:03 &                          331.404678 &                           -56.351045 &                                0.07000000029802322 &                                0.09000000357627869 &                                0.16899999976158142 &                              0.0010000000474974513 \\
                           1 &                               SB9287\_island\_117778 &                           SB9287\_component\_117778a &                                     J201136-511906 &                                 20:11:36.4 &                               -51:19:06 &                          302.901765 &                           -51.318587 &                                0.05000000074505806 &                                0.11999999731779099 &                                               0.25 &                              0.0020000000949949026 \\
                           1 &                               SB9287\_island\_120169 &                           SB9287\_component\_120169a &                                     J212505-512441 &                                 21:25:05.1 &                               -51:24:41 &                          321.271063 &                           -51.411491 &                               0.029999999329447746 &                                0.03999999910593033 &                                0.24699999392032623 &                              0.0010000000474974513 \\
                           1 &                                SB9287\_island\_47043 &                            SB9287\_component\_47043a &                                     J201310-595507 &                                 20:13:10.7 &                               -59:55:07 &                          303.294736 &                           -59.918677 &                                0.03999999910593033 &                                0.03999999910593033 &                                 0.5740000009536743 &                               0.003000000026077032 \\
                           1 &                               SB9287\_island\_115548 &                           SB9287\_component\_115548a &                                     J204920-505100 &                                 20:49:20.5 &                               -50:51:00 &                          312.335276 &                           -50.850061 &                                0.05000000074505806 &                                0.05999999865889549 &                                0.25200000405311584 &                              0.0010000000474974513 \\
                           1 &                               SB9287\_island\_183758 &                           SB9287\_component\_183758a &                                     J220721-520613 &                                 22:07:21.9 &                               -52:06:13 &                           331.84127 &                           -52.103833 &                               0.019999999552965164 &                               0.019999999552965164 &                                 0.1599999964237213 &                                                0.0 \\
                           1 &                               SB9287\_island\_115530 &                           SB9287\_component\_115530a &                                     J215029-544433 &                                 21:50:29.7 &                               -54:44:33 &                          327.623713 &                           -54.742522 &                               0.019999999552965164 &                               0.019999999552965164 &                                0.25600001215934753 &                              0.0010000000474974513 \\
                           1 &                                SB9287\_island\_42838 &                            SB9287\_component\_42838a &                                     J202631-511808 &                                 20:26:31.0 &                               -51:18:08 &                          306.629324 &                           -51.302429 &                                0.03999999910593033 &                                0.03999999910593033 &                                 0.6389999985694885 &                               0.003000000026077032 \\
                           1 &                                SB9287\_island\_95052 &                            SB9287\_component\_95052a &                                     J214245-612951 &                                 21:42:45.0 &                               -61:29:51 &                          325.687392 &                           -61.497613 &                                0.03999999910593033 &                                0.03999999910593033 &                                 0.3050000071525574 &                              0.0020000000949949026 \\
                           1 &                                 SB9287\_island\_5386 &                             SB9287\_component\_5386a &                                     J210052-531753 &                                 21:00:52.2 &                               -53:17:53 &                          315.217468 &                           -53.298196 &                                                0.0 &                                                0.0 &                                  9.277000427246094 &                               0.004999999888241291 \\
                           1 &                                SB9287\_island\_22774 &                            SB9287\_component\_22774b &                                     J205751-585022 &                                 20:57:51.9 &                               -58:50:22 &                          314.466434 &                           -58.839459 &                                0.05000000074505806 &                                0.05999999865889549 &                                 0.3050000071525574 &                              0.0020000000949949026 \\
                           1 &                                SB9287\_island\_47378 &                            SB9287\_component\_47378a &                                     J212126-603945 &                                 21:21:26.7 &                               -60:39:45 &                          320.361182 &                           -60.662562 &                               0.029999999329447746 &                               0.029999999329447746 &                                 0.5839999914169312 &                              0.0020000000949949026 \\
                           1 &                               SB9287\_island\_163833 &                           SB9287\_component\_163833a &                                     J202534-495354 &                                 20:25:34.8 &                               -49:53:54 &                          306.395117 &                           -49.898578 &                                0.03999999910593033 &                                0.03999999910593033 &                                0.18700000643730164 &                              0.0010000000474974513 \\
                           1 &                                SB9287\_island\_63905 &                            SB9287\_component\_63905a &                                     J210955-503036 &                                 21:09:55.7 &                               -50:30:36 &                          317.481933 &                           -50.510276 &                                0.09000000357627869 &                                0.07999999821186066 &                                0.42500001192092896 &                               0.004999999888241291 \\
                           1 &                               SB9287\_island\_145932 &                           SB9287\_component\_145932a &                                     J215707-513636 &                                 21:57:07.9 &                               -51:36:36 &                          329.282755 &                           -51.610035 &                               0.019999999552965164 &                               0.019999999552965164 &                                0.21199999749660492 &                              0.0010000000474974513 \\
\bottomrule
\end{tabular}


==> tables/table_3.tex <==
\begin{tabular}{lllllrrrrrrr}
\toprule
                                   selavy\_flux\_int &                                selavy\_flux\_int\_err &                            selavy\_spectral\_index &            wise\_source\_id &       wise\_source\_name &    wise\_ra &   wise\_dec &  w1mag &  w1sigm &  w2mag &  w2sigm &  wise\_separation \\
\midrule
                                0.4059999883174896 &                                0.02199999988079071 &                              -1.8200000524520874 & 3081m591\_b0-006425        & J203428.90-583929.6    & 308.620420 & -58.658238 & 15.117 &   0.021 & 14.874 &   0.056 &         7.579288 \\
[0.45500001311302185, 0.7770000100135803, 0.527... & [0.00800000037997961, 0.00800000037997961, 0.00... & [-1.5, -1.3700000047683716, -2.6700000762939453] & 3165m546\_b0-064532        & J210449.26-544655.9    & 316.205278 & -54.782197 & 15.949 &   0.038 & 15.890 &   0.107 &         6.362181 \\
                                 7.117000102996826 &                               0.012000000104308128 &                             -0.09000000357627869 & 3060m606\_b0-015305        & J202025.53-604829.1    & 305.106383 & -60.808099 & 16.132 &   0.044 & 15.668 &   0.098 &         0.741041 \\
                                 2.802999973297119 &                               0.014999999664723873 &                             -0.47999998927116394 & 3030m606\_b0-002266        & J201051.70-604908.9    & 302.715426 & -60.819157 & 13.546 &   0.008 & 13.484 &   0.013 &         3.546899 \\
                               0.23000000417232513 &                               0.004000000189989805 &                              -3.0399999618530273 & 3340m591\_b0-013331        & J221710.02-591718.9    & 334.291763 & -59.288604 & 16.264 &   0.047 & 15.648 &   0.092 &         2.458297 \\
                                0.3529999852180481 &                               0.010999999940395355 &                              -2.0399999618530273 & 3180m531\_b0-028843        & J211548.39-530857.9    & 318.951624 & -53.149422 & 16.899 &   0.100 & 16.999 &   0.373 &         9.248773 \\
                               0.17499999701976776 &                               0.004999999888241291 &                               -1.850000023841858 & 3094m621\_b0-081720        & J203404.97-622457.9    & 308.520729 & -62.416109 & 18.473 &   0.287 & 17.222 &     NaN &         2.024901 \\
                               0.21299999952316284 &                               0.003000000026077032 &                             -0.18000000715255737 & 3321m500\_b0-020432        & J220545.74-502550.4    & 331.440582 & -50.430686 & 16.784 &   0.086 & 16.685 &   0.307 &         1.158385 \\
                                0.5839999914169312 &                               0.017000000923871994 &                               -3.049999952316284 & 3321m500\_b0-037673        & J220957.54-493725.9    & 332.489758 & -49.623885 & 17.187 &   0.093 & 17.696 &   0.515 &         4.043253 \\
                                 0.328000009059906 &                               0.012000000104308128 &                               -2.200000047683716 & 3306m561\_b0-006465        & J215754.29-561005.9    & 329.476210 & -56.168321 & 15.341 &   0.017 & 15.052 &   0.046 &         1.155401 \\
                               0.19099999964237213 &                               0.003000000026077032 &                              -2.0999999046325684 & 3075m515\_b0-072008        & J203011.01-513906.5    & 307.545886 & -51.651830 & 17.082 &   0.158 & 17.195 &   0.428 &         6.603805 \\
                               0.22300000488758087 &                              0.0010000000474974513 &                               -4.059999942779541 & 3268m546\_b0-009395        & J215126.71-541419.8    & 327.861320 & -54.238857 & 16.015 &   0.046 & 15.401 &   0.060 &         0.879417 \\
                                0.1899999976158142 &                              0.0020000000949949026 &                             -0.49000000953674316 & 3283m591\_b0-004584        & J214905.79-583403.0    & 327.274146 & -58.567517 & 15.176 &   0.019 & 14.728 &   0.040 &         2.127142 \\
                               0.15700000524520874 &                              0.0010000000474974513 &                               -2.890000104904175 & 3191m546\_b0-043004        & J211916.51-544326.0    & 319.818794 & -54.723896 & 16.218 &   0.045 & 16.018 &   0.117 &         2.213328 \\
                                 1.222000002861023 &                               0.004999999888241291 &                             -0.12999999523162842 & 3126m621\_b0-002723        & J205252.59-621231.8    & 313.219144 & -62.208834 & 13.784 &   0.007 & 13.691 &   0.014 &         0.414304 \\
                               0.15199999511241913 &                              0.0020000000949949026 &                             0.019999999552965164 & 3168m591\_b0-056290        & J210642.23-583553.1    & 316.675962 & -58.598110 & 17.081 &   0.078 & 16.585 &   0.167 &         6.022324 \\
                                 4.288000106811523 &                               0.014000000432133675 &                              -0.3700000047683716 & 3350m576\_b0-015324        & J221750.05-581022.5    & 334.458567 & -58.172928 & 15.982 &   0.031 & 16.091 &   0.115 &         0.230795 \\
                               0.19900000095367432 &                              0.0010000000474974513 &                                -4.21999979019165 & 3306m561\_b0-041343        & J215806.53-562500.2    & 329.527206 & -56.416723 & 16.565 &   0.049 & 16.366 &   0.151 &        14.260636 \\
                                0.4300000071525574 &                               0.003000000026077032 &                              -1.3200000524520874 & 3333m561\_b0-007229        & J221455.56-552439.5    & 333.731537 & -55.410974 & 15.514 &   0.022 & 15.798 &   0.113 &         2.632653 \\
                                0.2809999883174896 &                              0.0010000000474974513 &                              -1.8700000047683716 & 3212m576\_b0-007986        & J212155.84-575238.7    & 320.482685 & -57.877437 & 15.231 &   0.019 & 15.308 &   0.054 &         0.540459 \\
                                 0.257999986410141 &                              0.0020000000949949026 &                             -0.05999999865889549 & 3081m591\_b0-018438        & J203015.83-591218.8    & 307.565992 & -59.205226 & 14.978 &   0.025 & 14.801 &   0.038 &         4.043800 \\
                               0.36399999260902405 &                              0.0020000000949949026 &                               -2.819999933242798 & 3194m515\_b0-007103        & J211617.92-512746.8    & 319.074705 & -51.463009 & 15.466 &   0.020 & 15.660 &   0.106 &         1.584045 \\
                               0.21699999272823334 &                              0.0020000000949949026 &                              -2.6500000953674316 & 3180m606\_b0-022010        & J211258.95-600829.8    & 318.245649 & -60.141622 & 16.675 &   0.052 & 16.379 &   0.169 &         1.026879 \\
                                 0.289000004529953 &                               0.003000000026077032 &                              -1.3700000047683716 & 3060m606\_b0-034126        & J202826.46-604527.0    & 307.110248 & -60.757519 & 15.644 &   0.025 & 15.524 &   0.098 &         3.667535 \\
                               0.20399999618530273 &                              0.0020000000949949026 &                              -1.2300000190734863 & 3337m515\_b0-020324        & J221430.16-514834.3    & 333.625696 & -51.809546 & 16.746 &   0.082 & 15.821 &   0.121 &         2.604921 \\
                                14.508999824523926 &                                0.00800000037997961 &                               -0.699999988079071 & 3170m515\_b0-009752        & J210804.38-505450.9    & 317.018259 & -50.914151 & 15.306 &   0.019 & 15.272 &   0.071 &         0.153555 \\
                                 0.164000004529953 &                              0.0020000000949949026 &                              -3.3299999237060547 & 3194m515\_b0-041701        & J211410.03-515337.5    & 318.541818 & -51.893757 & 17.493 &   0.111 & 16.820 &   0.275 &         2.352359 \\
                                 8.142999649047852 &                               0.008999999612569809 &                              -0.2199999988079071 & 3008m531\_b0-002952        & J200756.54-530903.8    & 301.985591 & -53.151081 & 13.983 &   0.010 & 12.968 &   0.011 &         0.419710 \\
                                0.1889999955892563 &                              0.0020000000949949026 &                               1.2599999904632568 & 3228m500\_b0-028240        & J212725.51-504101.4    & 321.856293 & -50.683726 & 16.925 &   0.096 & 16.792 &   0.214 &         6.675121 \\
                                0.1550000011920929 &                              0.0020000000949949026 &                                -5.03000020980835 & 3212m576\_b0-026499        & J212137.71-573450.6    & 320.407139 & -57.580732 & 16.869 &   0.064 & 17.320 &   0.332 &         5.384299 \\
                                2.7100000381469727 &                               0.003000000026077032 &                             -0.47999998927116394 & 3123m515\_b0-008525        & J204815.47-513211.7    & 312.064473 & -51.536587 & 15.081 &   0.018 & 14.976 &   0.048 &         1.223538 \\
                               0.32499998807907104 &                               0.003000000026077032 &                              -1.8799999952316284 & 3168m591\_b0-012035        & J210744.54-592851.2    & 316.935618 & -59.480891 & 15.255 &   0.016 & 15.275 &   0.053 &         4.115125 \\
                                0.2280000001192093 &                               0.008999999612569809 &                              -2.2100000381469727 & 3051m515\_b0-041950        & J201954.14-514141.6    & 304.975593 & -51.694912 & 16.491 &   0.058 & 17.020 &   0.320 &        19.015473 \\
                                0.2939999997615814 &                               0.003000000026077032 &                              -1.5399999618530273 & 3329m485\_b0-006032        & J221337.95-485036.4    & 333.408156 & -48.843466 & 15.305 &   0.019 & 14.906 &   0.050 &         0.318378 \\
                               0.10700000077486038 &                              0.0020000000949949026 &                               0.9599999785423279 & 3093m561\_b0-075209        & J203815.61-562656.8    & 309.565050 & -56.449130 & 16.942 &   0.105 & 17.171 &     NaN &         2.648265 \\
                               0.13199999928474426 &                              0.0020000000949949026 &                               3.1600000858306885 & 3089m546\_b0-001055        & J204010.59-550502.5    & 310.044162 & -55.084048 & 12.885 &   0.007 & 12.946 &   0.013 &        21.353130 \\
                               0.15700000524520874 &                              0.0020000000949949026 &                               -3.140000104904175 & 3295m576\_b0-004540        & J215753.87-572734.1    & 329.474477 & -57.459485 & 15.067 &   0.017 & 14.853 &   0.057 &         2.011420 \\
                               0.23399999737739563 &                              0.0010000000474974513 &                              -1.7200000286102295 & 3254m531\_b0-025726        & J214544.41-532821.4    & 326.435050 & -53.472611 & 16.901 &   0.076 & 16.258 &   0.131 &         1.353315 \\
                                 0.414000004529953 &                               0.003000000026077032 &                               -2.180000066757202 & 3221m621\_b0-007766        & J213251.55-614021.9    & 323.214831 & -61.672764 & 15.382 &   0.024 & 15.147 &   0.062 &         0.548053 \\
                                1.2009999752044678 &                               0.017000000923871994 &                              -0.7099999785423279 & 3170m515\_b0-003112        & J211247.94-512451.4    & 318.199784 & -51.414278 & 14.378 &   0.011 & 13.772 &   0.016 &         0.877056 \\
                                0.5709999799728394 &                              0.0020000000949949026 &                             -0.11999999731779099 & 3328m531\_b0-040148        & J220711.39-531741.3    & 331.797461 & -53.294824 & 17.959 &   0.249 & 16.524 &   0.196 &         1.268413 \\
                                0.5640000104904175 &                               0.003000000026077032 &                                             -2.0 & 3168m591\_b0-006548        & J211025.42-583054.5    & 317.605925 & -58.515166 & 14.555 &   0.010 & 14.199 &   0.022 &         2.113484 \\
                                0.1899999976158142 &                               0.004000000189989805 &                               -1.399999976158142 & 3135m500\_b0-017547        & J205245.77-492527.8    & 313.190726 & -49.424405 & 15.813 &   0.028 & 15.638 &   0.087 &         2.514752 \\
                                1.2510000467300415 &                               0.007000000216066837 &                               -0.800000011920929 & 3269m637\_b0-021587        & J215140.31-630101.1    & 327.917979 & -63.016994 & 16.992 &   0.143 & 17.419 &     NaN &        10.530239 \\
                                0.3070000112056732 &                              0.0020000000949949026 &                               -2.799999952316284 & 3065m500\_b0-023548        & J202618.87-495343.1    & 306.578642 & -49.895311 & 15.920 &   0.041 & 15.510 &   0.074 &         0.313349 \\
                                0.1979999989271164 &                               0.004000000189989805 &                               -2.940000057220459 & 3306m561\_b0-029379        & J220537.04-562103.0    & 331.404362 & -56.350836 & 16.618 &   0.051 & 16.371 &   0.171 &         0.754684 \\
                               0.24899999797344208 &                               0.003000000026077032 &                              0.05999999865889549 & 3027m515\_b0-041954        & J201136.70-511907.0    & 302.902938 & -51.318633 & 15.158 &   0.019 & 15.160 &   0.049 &         2.520252 \\
                               0.22599999606609344 &                              0.0020000000949949026 &                              -1.7599999904632568 & 3218m515\_b0-007502        & J212505.27-512441.9    & 321.271977 & -51.411646 & 15.591 &   0.025 & 15.411 &   0.063 &         2.205200 \\
                                0.6299999952316284 &                               0.006000000052154064 &                              -1.5700000524520874 & 3030m606\_b0-066638        & J201310.65-595505.3    & 303.294375 & -59.918161 & 15.660 &   0.056 & 14.730 &     NaN &         1.719619 \\
                                0.2540000081062317 &                              0.0020000000949949026 &                               -1.159999966621399 & 3123m515\_b0-025394        & J204920.49-505059.7    & 312.335407 & -50.849933 & 16.554 &   0.059 & 16.362 &   0.211 &         0.362941 \\
                               0.13300000131130219 &                              0.0010000000474974513 &                               -2.299999952316284 & 3313m515\_b0-012966        & J220722.09-520611.9    & 331.842081 & -52.103309 & 16.205 &   0.045 & 16.120 &   0.122 &         2.312164 \\
                               0.25999999046325684 &                              0.0010000000474974513 &                               -2.869999885559082 & 3268m546\_b0-035772        & J215029.78-544434.6    & 327.624114 & -54.742967 & 16.109 &   0.039 & 15.773 &   0.094 &         2.294895 \\
                                0.7639999985694885 &                               0.004999999888241291 &                              -1.3300000429153442 & 3075m515\_b0-084722        & J202630.81-511808.0    & 306.628394 & -51.302232 & 16.457 &   0.053 & 16.490 &   0.193 &         2.125119 \\
                                0.2680000066757202 &                              0.0020000000949949026 &                              -0.3499999940395355 & 3252m621\_b0-067403        & J214245.60-612945.7    & 325.690031 & -61.496032 & 17.393 &   0.102 & 17.843 &     NaN &         7.005852 \\
                                10.543000221252441 &                                0.00800000037997961 &                              -0.9200000166893005 & 3156m531\_b0-018882        & J210052.27-531753.4    & 315.217796 & -53.298192 & 16.336 &   0.060 & 16.312 &   0.151 &         0.844946 \\
                               0.29600000381469727 &                               0.004000000189989805 &                              -1.9299999475479126 & 3139m591\_b0-012179        & J205752.02-585021.7    & 314.466777 & -58.839361 & 15.545 &   0.025 & 14.884 &   0.045 &         0.757527 \\
                                0.5649999976158142 &                               0.003000000026077032 &                              -1.3700000047683716 & 3210m606\_b0-011670        & J212126.61-603945.4    & 320.360874 & -60.662621 & 15.708 &   0.023 & 15.292 &   0.055 &         0.717968 \\
                               0.16899999976158142 &                              0.0020000000949949026 &                              -2.0899999141693115 & 3065m500\_b0-009987        & J202534.82-495354.0    & 306.395110 & -49.898334 & 15.257 &   0.019 & 15.177 &   0.067 &         0.600615 \\
                                0.3720000088214874 &                               0.007000000216066837 &                              -0.3499999940395355 & 3181m500\_b0-043828        & J210955.77-503035.8    & 317.482414 & -50.509966 & 16.961 &   0.073 & 17.122 &   0.310 &         1.424621 \\
                               0.19900000095367432 &                              0.0010000000474974513 &                              -1.9700000286102295 & 3290m515\_b0-003910        & J215708.03-513636.2    & 329.283466 & -51.610079 & 15.151 &   0.019 & 14.856 &   0.044 &         1.980619 \\
\bottomrule
\end{tabular}


==> tables/table_4.tex <==
\begin{tabular}{rrrrrrrrrrrr}
\toprule
 des\_coadd\_object\_id &     des\_ra &    des\_dec &  des\_mag\_auto\_g &  des\_magerr\_auto\_g &  des\_mag\_auto\_r &  des\_magerr\_auto\_r &  des\_mag\_auto\_i &  des\_magerr\_auto\_i &  des\_mag\_auto\_z &  des\_magerr\_auto\_z &  des\_mag\_auto\_y \\
\midrule
           891204709 & 308.620442 & -58.658253 &         20.1560 &           0.007718 &         18.9599 &           0.003791 &         18.5023 &           0.004540 &         18.1542 &           0.005820 &         18.1015 \\
           906717097 & 316.205705 & -54.781718 &         24.6290 &           0.297892 &         23.8668 &           0.202265 &         23.1804 &           0.194136 &         23.2228 &           0.362313 &         23.0781 \\
           894418836 & 305.106488 & -60.808020 &         24.5747 &           0.396818 &         22.8444 &           0.115846 &         21.7558 &           0.065487 &         20.8517 &           0.058129 &         20.8238 \\
           870669166 & 302.792386 & -61.021167 &         25.0755 &           0.466038 &         99.0000 &          99.000000 &         23.6292 &           0.279397 &         23.6093 &           0.483738 &         24.7094 \\
          1698370300 & 334.291805 & -59.288600 &         25.2507 &           0.479291 &         22.9624 &           0.077562 &         21.5085 &           0.036307 &         21.0220 &           0.042048 &         21.0460 \\
           912575550 & 318.951639 & -53.149208 &         22.5815 &           0.037681 &         21.6325 &           0.023850 &         21.1924 &           0.027049 &         20.9183 &           0.042374 &         21.1707 \\
           893973374 & 308.520453 & -62.416146 &         24.1130 &           0.205375 &         23.2628 &           0.138177 &         23.0371 &           0.200309 &         22.2223 &           0.183545 &         23.3995 \\
           949050269 & 331.440323 & -50.430582 &         23.9684 &           0.164714 &         22.9879 &           0.087547 &         22.2543 &           0.087334 &         21.5678 &           0.081669 &         21.3706 \\
           951834284 & 332.489962 & -49.624265 &         24.4043 &           0.183055 &         22.7524 &           0.054401 &         21.9632 &           0.043572 &         21.6767 &           0.058901 &         21.4425 \\
           942207571 & 329.476271 & -56.168356 &         20.4628 &           0.011425 &         19.3850 &           0.005843 &         18.9059 &           0.006121 &         18.6260 &           0.008889 &         18.5192 \\
           893720751 & 307.545121 & -51.652137 &         23.9784 &           0.141877 &         22.9504 &           0.073536 &         21.4462 &           0.035561 &         20.7744 &           0.033333 &         20.7643 \\
           938691641 & 327.861487 & -54.238871 &         23.6850 &           0.157211 &         22.6138 &           0.074669 &         21.5935 &           0.050351 &         20.8141 &           0.048207 &         20.7547 \\
           936661831 & 327.274179 & -58.567515 &         20.8344 &           0.007922 &         19.4301 &           0.002947 &         18.9587 &           0.003621 &         18.6274 &           0.005421 &         18.5689 \\
           915804436 & 319.819006 & -54.723858 &         24.7386 &           0.344542 &         23.6961 &           0.182152 &         22.8938 &           0.146847 &         22.4631 &           0.198228 &         22.7550 \\
           882841759 & 313.219066 & -62.208820 &         17.7926 &           0.002051 &         16.8465 &           0.001135 &         16.4373 &           0.001351 &         16.1447 &           0.002015 &         16.0187 \\
           906803330 & 316.676085 & -58.597933 &         24.3689 &           0.158777 &         23.8916 &           0.153743 &         23.4029 &           0.170696 &         23.2011 &           0.251188 &         23.0214 \\
          1698747670 & 334.458562 & -58.172833 &         23.3873 &           0.162746 &         22.1649 &           0.067526 &         21.2313 &           0.048897 &         20.7077 &           0.059016 &         20.5977 \\
           942233808 & 329.527125 & -56.416660 &         22.4223 &           0.030711 &         21.3382 &           0.015876 &         20.9794 &           0.017631 &         20.6790 &           0.028227 &         20.9701 \\
           953964843 & 333.731618 & -55.410998 &         23.7228 &           0.105747 &         21.5237 &           0.022901 &         20.3250 &           0.011599 &         19.8266 &           0.015595 &         19.7065 \\
           917215732 & 320.482766 & -57.877401 &         22.0972 &           0.044289 &         20.2641 &           0.010769 &         19.4825 &           0.009576 &         19.1081 &           0.012570 &         19.0510 \\
           891650532 & 307.566200 & -59.205177 &         21.4325 &           0.030294 &         20.2484 &           0.013903 &         19.7623 &           0.017545 &         19.3782 &           0.017761 &         19.2737 \\
           914908096 & 319.074695 & -51.463055 &         23.1885 &           0.084946 &         21.5534 &           0.029528 &         20.7522 &           0.024481 &         20.3641 &           0.032111 &         20.0089 \\
           909871635 & 318.245761 & -60.141687 &         22.2525 &           0.023581 &         21.9337 &           0.029757 &         21.3153 &           0.028973 &         20.9588 &           0.037356 &         20.8265 \\
           896631660 & 307.110379 & -60.757911 &         22.5560 &           0.067333 &         22.1028 &           0.062069 &         21.6061 &           0.067601 &         21.1141 &           0.075863 &         21.6526 \\
           952863736 & 333.625912 & -51.809077 &         26.7139 &           0.777749 &         26.6027 &           0.958280 &         26.6515 &           1.596880 &         24.2804 &           0.370205 &         23.8001 \\
           906250843 & 317.018209 & -50.914184 &         23.3517 &           0.168047 &         21.4947 &           0.045996 &         20.4346 &           0.029731 &         19.8506 &           0.033227 &         19.8224 \\
           910549486 & 318.541803 & -51.893847 &         24.0370 &           0.109169 &         23.4368 &           0.099542 &         23.5873 &           0.184722 &         23.4181 &           0.302915 &         22.6714 \\
           900293883 & 301.985604 & -53.151112 &         19.3676 &           0.002488 &         19.0318 &           0.002525 &         18.7167 &           0.003223 &         18.4385 &           0.004480 &         18.4666 \\
           922791721 & 321.855974 & -50.683528 &         25.6007 &           0.501675 &         24.9073 &           0.394352 &         23.5152 &           0.190054 &         22.7954 &           0.169182 &         22.9282 \\
           917186581 & 320.407166 & -57.580811 &         22.8966 &           0.056295 &         21.1458 &           0.015829 &         20.5343 &           0.016312 &         20.2118 &           0.019799 &         20.0341 \\
           881304714 & 312.064558 & -51.536745 &         21.9919 &           0.048432 &         19.9134 &           0.010669 &         19.1327 &           0.008828 &         18.7356 &           0.011571 &         18.6603 \\
           907242703 & 316.935692 & -59.480839 &         23.0187 &           0.080260 &         21.7920 &           0.037854 &         20.9962 &           0.031900 &         20.8020 &           0.045608 &         20.8510 \\
           876543208 & 304.975676 & -51.695046 &         23.6588 &           0.118065 &         22.1938 &           0.040894 &         21.4988 &           0.035019 &         21.0832 &           0.046109 &         21.1580 \\
           952988465 & 333.408250 & -48.843498 &         20.7329 &           0.013790 &         19.7257 &           0.006467 &         19.3405 &           0.008355 &         18.9844 &           0.010614 &         19.0513 \\
           895639661 & 309.567131 & -56.449201 &         23.3984 &           0.108852 &         23.0477 &           0.084559 &         22.9002 &           0.135492 &         22.6851 &           0.217507 &         24.2407 \\
           895565755 & 310.044213 & -55.084102 &         14.9899 &           0.000186 &         17.2419 &           0.001484 &         17.0984 &           0.002164 &         16.9088 &           0.003593 &         14.0627 \\
           944407818 & 329.474465 & -57.459467 &         20.6638 &           0.010268 &         19.3296 &           0.004392 &         18.8710 &           0.004626 &         18.5282 &           0.007068 &         18.4375 \\
           935707766 & 326.435031 & -53.472600 &         23.6053 &           0.100978 &         23.1581 &           0.089460 &         22.7574 &           0.117134 &         21.9926 &           0.117980 &         22.1153 \\
           925968999 & 323.214853 & -61.672784 &         21.8373 &           0.024424 &         20.2528 &           0.008415 &         19.7423 &           0.008969 &         19.3970 &           0.011694 &         19.2559 \\
           911712308 & 318.199842 & -51.414287 &         19.9304 &           0.006970 &         18.9082 &           0.004049 &         18.3191 &           0.004124 &         18.0470 &           0.005464 &         17.9366 \\
           948910003 & 331.797413 & -53.294969 &         24.0283 &           0.127244 &         23.4789 &           0.111756 &         22.8125 &           0.095221 &         22.2629 &           0.111531 &         22.3571 \\
           908419763 & 317.606027 & -58.515087 &         19.2450 &           0.002760 &         18.5499 &           0.002168 &         18.1993 &           0.002766 &         18.0435 &           0.004272 &         17.9934 \\
           883391706 & 313.191013 & -49.424630 &         22.6730 &           0.067285 &         21.3571 &           0.029075 &         20.8804 &           0.034600 &         20.4803 &           0.040614 &         20.1791 \\
           940525300 & 327.917921 & -63.016990 &         24.0935 &           0.140028 &         22.1928 &           0.033325 &         21.3534 &           0.027002 &         21.0016 &           0.040778 &         21.0385 \\
           889388909 & 306.578870 & -49.895325 &         25.5815 &           0.476837 &         24.2422 &           0.181762 &         23.2895 &           0.133815 &         22.6978 &           0.179063 &         23.0324 \\
           949400634 & 331.404447 & -56.350654 &         23.8359 &           0.166303 &         23.3229 &           0.150488 &         22.8329 &           0.160911 &         22.5412 &           0.204291 &         24.2645 \\
           893338638 & 302.899858 & -51.318519 &         25.8994 &           0.570354 &         24.5106 &           0.237199 &         23.8450 &           0.222590 &         23.5167 &           0.295048 &         99.0000 \\
           918894707 & 321.272325 & -51.411765 &         20.4186 &           0.006794 &         19.1470 &           0.003115 &         18.6344 &           0.003070 &         18.3647 &           0.004625 &         18.2904 \\
           872120983 & 303.294202 & -59.918487 &         23.0158 &           0.050529 &         23.0757 &           0.096509 &         23.0183 &           0.120925 &         22.7913 &           0.250810 &         22.8169 \\
           882524452 & 312.334839 & -50.850026 &         24.4685 &           0.280054 &         24.1847 &           0.292445 &         23.2336 &           0.198735 &         22.5859 &           0.196503 &         22.0352 \\
           950070819 & 331.842061 & -52.103259 &         25.2610 &           0.603275 &         23.4666 &           0.179362 &         22.1618 &           0.081246 &         21.4563 &           0.075316 &         21.6351 \\
           937719072 & 327.624262 & -54.743044 &         23.0074 &           0.092032 &         22.1057 &           0.058258 &         21.4925 &           0.051952 &         20.9639 &           0.068997 &         20.9136 \\
           893682392 & 306.628710 & -51.302138 &         24.7467 &           0.297058 &         23.8906 &           0.178513 &         23.2626 &           0.173541 &         22.4637 &           0.146857 &         22.2336 \\
           932546195 & 325.690681 & -61.496182 &         23.4715 &           0.068242 &         22.0762 &           0.025892 &         20.6953 &           0.011925 &         20.1531 &           0.015064 &         20.0273 \\
           902373378 & 315.217759 & -53.298223 &         23.7848 &           0.118254 &         22.3476 &           0.045978 &         21.4647 &           0.033280 &         20.8763 &           0.043187 &         21.0149 \\
           902210404 & 314.466801 & -58.839389 &         22.8754 &           0.074286 &         21.5343 &           0.030698 &         20.6650 &           0.025519 &         20.3596 &           0.038719 &         20.2761 \\
           916979726 & 320.360822 & -60.662559 &         24.7308 &           0.310994 &         23.3738 &           0.127043 &         21.8109 &           0.054812 &         21.2972 &           0.062709 &         21.2285 \\
           889388920 & 306.395081 & -49.898265 &         21.8962 &           0.026875 &         20.7563 &           0.012353 &         20.1467 &           0.013673 &         19.7454 &           0.018280 &         19.6122 \\
           910508533 & 317.482193 & -50.510178 &         23.8373 &           0.092737 &         23.5344 &           0.110963 &         23.0932 &           0.124792 &         22.6398 &           0.142224 &         23.2537 \\
           941129209 & 329.283499 & -51.610100 &         18.8084 &           0.002724 &         18.1912 &           0.002108 &         17.8818 &           0.002449 &         17.7117 &           0.003596 &         17.6549 \\
\bottomrule
\end{tabular}

